X-ray Emission of Nearby Low-mass and Sun-like Stars with Directly Imageable Habitable Zones

Stellar X-ray and UV radiation can significantly affect the survival, composition, and long-term evolution of the atmospheres of planets in or near their host star's habitable zone (HZ). Especially interesting are planetary systems in the solar neighborhood that may host temperate and potentially habitable surface conditions, which may be analyzed by future ground and space-based direct-imaging surveys for signatures of habitability and life. To advance our understanding of the radiation environment in these systems, we leverage $\sim$3 Msec of XMM-Newton and Chandra observations in order to measure three fundamental stellar properties at X-ray energies for 57 nearby FGKM stellar systems: the shape of the stellar X-ray spectrum, the luminosity, and the timescales over which the stars vary (e.g., due to flares). These systems possess HZs that will be directly imageable to next-generation telescopes such as the Habitable Worlds Observatory and ground-based Extremely Large Telescopes (ELTs). We identify 29 stellar systems with $L_X/L_{\rm bol}$ ratios similar to (or less than) that of the Sun; any potential planets in the habitable zones of these stars therefore reside in present day X-ray radiation environments similar to (or less hostile than) modern Earth, though a broader set of these targets could host habitable planets. An additional 19 stellar systems have been observed with the Swift X-ray Telescope; in total, only $\sim$30% of potential direct imaging target stars has been observed with XMM-Newton, Chandra, or Swift. The data products from this work (X-ray light curves and spectra) are available via a public Zenodo repository (doi: 10.5281/zenodo.11490574).

==> StarSections/GL892_subsection.tex <==
\subsection{GL 892}
Age estimates broadly agree: 11.0$\pm$2.2 Gyr \citep{Gillon+17} vs. 12.46 Gyr \citep{Turnbull15}. Hosts five confirmed exoplanets; the existence of a sixth exoplanet is controversial (HD 219134 f). HD 219134 b, c, d, g and h have masses of \mpsini\ $\sim$4.1 \MEarth with an orbital period $\sim$3 days ($\sim$0.04 AU), $\sim$3.5 \MEarth with an orbital period of $\sim$6.8 days ($\sim$0.06 AU), $\sim$16 \MEarth\ with an orbital period of $\sim$47 days ($\sim$0.2 AU), $\sim$11 \Mearth\ with an orbital period of $\sim$94 days ($\sim$0.37 AU), and $\sim$0.3 \MJup\ with an orbital period of $\sim$2100 days ($\sim$3 AU), respectively. Planetary data taken from \citet{Rosenthal+21,Gillon+17,Vogt+15}.

GL 892 was detected at $\sim$29$\sigma$ significance in a 30.8 ks \XMM/PN observation. No significant variability was observed in the X-ray light curve, and the star was well-described by a two-component thermal plasma model (see Figure Set~\ref{fig:LightCurves-FigureSet} and Table~\ref{table:spectral_modeling}).
